Large-scale cosmic ray anisotropies with 19 years of data from the Pierre Auger Observatory

Results are presented for the measurement of large-scale anisotropies in the arrival directions of ultra-high-energy cosmic rays detected at the Pierre Auger Observatory during 19 years of operation, prior to AugerPrime, the upgrade of the Observatory. The 3D dipole amplitude and direction are reconstructed above $4\,$EeV in four energy bins. Besides the established dipolar anisotropy in right ascension above $8\,$EeV, the Fourier amplitude of the $8$ to $16\,$EeV energy bin is now also above the $5\sigma$ discovery level. No time variation of the dipole moment above $8\,$EeV is found, setting an upper limit to the rate of change of such variations of $0.3\%$ per year at the $95\%$ confidence level. Additionally, the results for the angular power spectrum are shown, demonstrating no other statistically significant multipoles. The results for the equatorial dipole component down to $0.03\,$EeV are presented, using for the first time a data set obtained with a trigger that has been optimized for lower energies. Finally, model predictions are discussed and compared with observations, based on two source emission scenarios obtained in the combined fit of spectrum and composition above $0.6\,$EeV.

==> aastex_authorlist.tex <==
% created on 2024-08-07
\author{A.~Abdul Halim}
\affiliation{University of Adelaide, Adelaide, S.A., Australia}

\author{P.~Abreu}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{M.~Aglietta}
\affiliation{Osservatorio Astrofisico di Torino (INAF), Torino, Italy}
\affiliation{INFN, Sezione di Torino, Torino, Italy}

\author{I.~Allekotte}
\affiliation{Centro At\'omico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), San Carlos de Bariloche, Argentina}

\author{K.~Almeida Cheminant}
\affiliation{Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}

\author{A.~Almela}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\affiliation{Universidad Tecnol\'ogica Nacional -- Facultad Regional Buenos Aires, Buenos Aires, Argentina}

\author{R.~Aloisio}
\affiliation{Gran Sasso Science Institute, L'Aquila, Italy}
\affiliation{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}

\author{J.~Alvarez-Mu\~niz}
\affiliation{Instituto Galego de F\'\i{}sica de Altas Enerx\'\i{}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain}

\author{A.~Ambrosone}
\affiliation{Gran Sasso Science Institute, L'Aquila, Italy}

\author{J.~Ammerman Yebra}
\affiliation{Instituto Galego de F\'\i{}sica de Altas Enerx\'\i{}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain}

\author{G.A.~Anastasi}
\affiliation{Universit\`a di Catania, Dipartimento di Fisica e Astronomia ``Ettore Majorana``, Catania, Italy}
\affiliation{INFN, Sezione di Catania, Catania, Italy}

\author{L.~Anchordoqui}
\affiliation{Department of Physics and Astronomy, Lehman College, City University of New York, Bronx, NY, USA}

\author{B.~Andrada}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{L.~Andrade Dourado}
\affiliation{Gran Sasso Science Institute, L'Aquila, Italy}
\affiliation{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}

\author{S.~Andringa}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{L.~Apollonio}
\affiliation{Universit\`a di Milano, Dipartimento di Fisica, Milano, Italy}
\affiliation{INFN, Sezione di Milano, Milano, Italy}

\author{C.~Aramo}
\affiliation{INFN, Sezione di Napoli, Napoli, Italy}

\author{P.R.~Ara\'ujo Ferreira}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{E.~Arnone}
\affiliation{Universit\`a Torino, Dipartimento di Fisica, Torino, Italy}
\affiliation{INFN, Sezione di Torino, Torino, Italy}

\author{J.C.~Arteaga Vel\'azquez}
\affiliation{Universidad Michoacana de San Nicol\'as de Hidalgo, Morelia, Michoac\'an, M\'exico}

\author{P.~Assis}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{G.~Avila}
\affiliation{Observatorio Pierre Auger and Comisi\'on Nacional de Energ\'\i{}a At\'omica, Malarg\"ue, Argentina}

\author{E.~Avocone}
\affiliation{Universit\`a dell'Aquila, Dipartimento di Scienze Fisiche e Chimiche, L'Aquila, Italy}
\affiliation{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}

\author{A.~Bakalova}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{F.~Barbato}
\affiliation{Gran Sasso Science Institute, L'Aquila, Italy}
\affiliation{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}

\author{A.~Bartz Mocellin}
\affiliation{Colorado School of Mines, Golden, CO, USA}

\author{J.A.~Bellido}
\affiliation{University of Adelaide, Adelaide, S.A., Australia}

\author{C.~Berat}
\affiliation{Univ.\ Grenoble Alpes, CNRS, Grenoble Institute of Engineering Univ.\ Grenoble Alpes, LPSC-IN2P3, 38000 Grenoble, France}

\author{M.E.~Bertaina}
\affiliation{Universit\`a Torino, Dipartimento di Fisica, Torino, Italy}
\affiliation{INFN, Sezione di Torino, Torino, Italy}

\author{G.~Bhatta}
\affiliation{Institute of Nuclear Physics PAN, Krakow, Poland}

\author{M.~Bianciotto}
\affiliation{Universit\`a Torino, Dipartimento di Fisica, Torino, Italy}
\affiliation{INFN, Sezione di Torino, Torino, Italy}

\author{P.L.~Biermann}
\altaffiliation{Max-Planck-Institut f\"ur Radioastronomie, Bonn, Germany}

\author{V.~Binet}
\affiliation{Instituto de F\'\i{}sica de Rosario (IFIR) -- CONICET/U.N.R.\ and Facultad de Ciencias Bioqu\'\i{}micas y Farmac\'euticas U.N.R., Rosario, Argentina}

\author{K.~Bismark}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Experimental Particle Physics, Karlsruhe, Germany}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{T.~Bister}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}
\affiliation{Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands}

\author{J.~Biteau}
\altaffiliation{Institut universitaire de France (IUF), France}
\affiliation{Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, Orsay, France}

\author{J.~Blazek}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{C.~Bleve}
\affiliation{Univ.\ Grenoble Alpes, CNRS, Grenoble Institute of Engineering Univ.\ Grenoble Alpes, LPSC-IN2P3, 38000 Grenoble, France}

\author{J.~Bl\"umer}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{M.~Boh\'a\v{c}ov\'a}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{D.~Boncioli}
\affiliation{Universit\`a dell'Aquila, Dipartimento di Scienze Fisiche e Chimiche, L'Aquila, Italy}
\affiliation{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}

\author{C.~Bonifazi}
\affiliation{International Center of Advanced Studies and Instituto de Ciencias F\'\i{}sicas, ECyT-UNSAM and CONICET, Campus Miguelete -- San Mart\'\i{}n, Buenos Aires, Argentina}

\author{L.~Bonneau Arbeletche}
\affiliation{Universidade Estadual de Campinas (UNICAMP), IFGW, Campinas, SP, Brazil}

\author{N.~Borodai}
\affiliation{Institute of Nuclear Physics PAN, Krakow, Poland}

\author{J.~Brack}
\altaffiliation{Colorado State University, Fort Collins, CO, USA}

\author{P.G.~Brichetto Orchera}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{F.L.~Briechle}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{A.~Bueno}
\affiliation{Universidad de Granada and C.A.F.P.E., Granada, Spain}

\author{S.~Buitink}
\affiliation{Vrije Universiteit Brussels, Brussels, Belgium}

\author{M.~Buscemi}
\affiliation{INFN, Sezione di Catania, Catania, Italy}
\affiliation{Universit\`a di Catania, Dipartimento di Fisica e Astronomia ``Ettore Majorana``, Catania, Italy}

\author{M.~B\"usken}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Experimental Particle Physics, Karlsruhe, Germany}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{A.~Bwembya}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}
\affiliation{Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands}

\author{K.S.~Caballero-Mora}
\affiliation{Universidad Aut\'onoma de Chiapas, Tuxtla Guti\'errez, Chiapas, M\'exico}

\author{S.~Cabana-Freire}
\affiliation{Instituto Galego de F\'\i{}sica de Altas Enerx\'\i{}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain}

\author{L.~Caccianiga}
\affiliation{Universit\`a di Milano, Dipartimento di Fisica, Milano, Italy}
\affiliation{INFN, Sezione di Milano, Milano, Italy}

\author{F.~Campuzano}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), and Universidad Tecnol\'ogica Nacional -- Facultad Regional Mendoza (CONICET/CNEA), Mendoza, Argentina}

\author{R.~Caruso}
\affiliation{Universit\`a di Catania, Dipartimento di Fisica e Astronomia ``Ettore Majorana``, Catania, Italy}
\affiliation{INFN, Sezione di Catania, Catania, Italy}

\author{A.~Castellina}
\affiliation{Osservatorio Astrofisico di Torino (INAF), Torino, Italy}
\affiliation{INFN, Sezione di Torino, Torino, Italy}

\author{F.~Catalani}
\affiliation{Universidade de S\~ao Paulo, Escola de Engenharia de Lorena, Lorena, SP, Brazil}

\author{G.~Cataldi}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{L.~Cazon}
\affiliation{Instituto Galego de F\'\i{}sica de Altas Enerx\'\i{}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain}

\author{M.~Cerda}
\affiliation{Observatorio Pierre Auger, Malarg\"ue, Argentina}

\author{B.~\v{C}erm\'akov\'a}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{A.~Cermenati}
\affiliation{Gran Sasso Science Institute, L'Aquila, Italy}
\affiliation{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}

\author{J.A.~Chinellato}
\affiliation{Universidade Estadual de Campinas (UNICAMP), IFGW, Campinas, SP, Brazil}

\author{J.~Chudoba}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{L.~Chytka}
\affiliation{Palacky University, Olomouc, Czech Republic}

\author{R.W.~Clay}
\affiliation{University of Adelaide, Adelaide, S.A., Australia}

\author{A.C.~Cobos Cerutti}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), and Universidad Tecnol\'ogica Nacional -- Facultad Regional Mendoza (CONICET/CNEA), Mendoza, Argentina}

\author{R.~Colalillo}
\affiliation{Universit\`a di Napoli ``Federico II'', Dipartimento di Fisica ``Ettore Pancini'', Napoli, Italy}
\affiliation{INFN, Sezione di Napoli, Napoli, Italy}

\author{R.~Concei\c{c}\~ao}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{A.~Condorelli}
\affiliation{Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, Orsay, France}

\author{G.~Consolati}
\affiliation{INFN, Sezione di Milano, Milano, Italy}
\affiliation{Politecnico di Milano, Dipartimento di Scienze e Tecnologie Aerospaziali , Milano, Italy}

\author{M.~Conte}
\affiliation{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{F.~Convenga}
\affiliation{Universit\`a dell'Aquila, Dipartimento di Scienze Fisiche e Chimiche, L'Aquila, Italy}
\affiliation{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}

\author{D.~Correia dos Santos}
\affiliation{Universidade Federal do Rio de Janeiro, Instituto de F\'\i{}sica, Rio de Janeiro, RJ, Brazil}

\author{P.J.~Costa}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{C.E.~Covault}
\affiliation{Case Western Reserve University, Cleveland, OH, USA}

\author{M.~Cristinziani}
\affiliation{Universit\"at Siegen, Department Physik -- Experimentelle Teilchenphysik, Siegen, Germany}

\author{C.S.~Cruz Sanchez}
\affiliation{IFLP, Universidad Nacional de La Plata and CONICET, La Plata, Argentina}

\author{S.~Dasso}
\affiliation{Instituto de Astronom\'\i{}a y F\'\i{}sica del Espacio (IAFE, CONICET-UBA), Buenos Aires, Argentina}
\affiliation{Departamento de F\'\i{}sica and Departamento de Ciencias de la Atm\'osfera y los Oc\'eanos, FCEyN, Universidad de Buenos Aires and CONICET, Buenos Aires, Argentina}

\author{K.~Daumiller}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{B.R.~Dawson}
\affiliation{University of Adelaide, Adelaide, S.A., Australia}

\author{R.M.~de Almeida}
\affiliation{Universidade Federal do Rio de Janeiro, Instituto de F\'\i{}sica, Rio de Janeiro, RJ, Brazil}

\author{B.~de Errico}
\affiliation{Universidade Federal do Rio de Janeiro, Instituto de F\'\i{}sica, Rio de Janeiro, RJ, Brazil}

\author{J.~de Jes\'us}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{S.J.~de Jong}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}
\affiliation{Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands}

\author{J.R.T.~de Mello Neto}
\affiliation{Universidade Federal do Rio de Janeiro, Instituto de F\'\i{}sica, Rio de Janeiro, RJ, Brazil}

\author{I.~De Mitri}
\affiliation{Gran Sasso Science Institute, L'Aquila, Italy}
\affiliation{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}

\author{J.~de Oliveira}
\affiliation{Instituto Federal de Educa\c{c}\~ao, Ci\^encia e Tecnologia do Rio de Janeiro (IFRJ), Brazil}

\author{D.~de Oliveira Franco}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{F.~de Palma}
\affiliation{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{V.~de Souza}
\affiliation{Universidade de S\~ao Paulo, Instituto de F\'\i{}sica de S\~ao Carlos, S\~ao Carlos, SP, Brazil}

\author{E.~De Vito}
\affiliation{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{A.~Del Popolo}
\affiliation{Universit\`a di Catania, Dipartimento di Fisica e Astronomia ``Ettore Majorana``, Catania, Italy}
\affiliation{INFN, Sezione di Catania, Catania, Italy}

\author{O.~Deligny}
\affiliation{CNRS/IN2P3, IJCLab, Universit\'e Paris-Saclay, Orsay, France}

\author{N.~Denner}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{L.~Deval}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{A.~di Matteo}
\affiliation{INFN, Sezione di Torino, Torino, Italy}

\author{C.~Dobrigkeit}
\affiliation{Universidade Estadual de Campinas (UNICAMP), IFGW, Campinas, SP, Brazil}

\author{J.C.~D'Olivo}
\affiliation{Universidad Nacional Aut\'onoma de M\'exico, M\'exico, D.F., M\'exico}

\author{L.M.~Domingues Mendes}
\affiliation{Centro Brasileiro de Pesquisas Fisicas, Rio de Janeiro, RJ, Brazil}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{Q.~Dorosti}
\affiliation{Universit\"at Siegen, Department Physik -- Experimentelle Teilchenphysik, Siegen, Germany}

\author{J.C.~dos Anjos}
\affiliation{Centro Brasileiro de Pesquisas Fisicas, Rio de Janeiro, RJ, Brazil}

\author{R.C.~dos Anjos}
\affiliation{Universidade Federal do Paran\'a, Setor Palotina, Palotina, Brazil}

\author{J.~Ebr}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{F.~Ellwanger}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{M.~Emam}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}
\affiliation{Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands}

\author{R.~Engel}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Experimental Particle Physics, Karlsruhe, Germany}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{I.~Epicoco}
\affiliation{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{M.~Erdmann}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{A.~Etchegoyen}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\affiliation{Universidad Tecnol\'ogica Nacional -- Facultad Regional Buenos Aires, Buenos Aires, Argentina}

\author{C.~Evoli}
\affiliation{Gran Sasso Science Institute, L'Aquila, Italy}
\affiliation{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}

\author{H.~Falcke}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}
\affiliation{Stichting Astronomisch Onderzoek in Nederland (ASTRON), Dwingeloo, The Netherlands}
\affiliation{Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands}

\author{G.~Farrar}
\affiliation{New York University, New York, NY, USA}

\author{A.C.~Fauth}
\affiliation{Universidade Estadual de Campinas (UNICAMP), IFGW, Campinas, SP, Brazil}

\author{T.~Fehler}
\affiliation{Universit\"at Siegen, Department Physik -- Experimentelle Teilchenphysik, Siegen, Germany}

\author{F.~Feldbusch}
\affiliation{Karlsruhe Institute of Technology (KIT), Institut f\"ur Prozessdatenverarbeitung und Elektronik, Karlsruhe, Germany}

\author{A.~Fernandes}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{B.~Fick}
\affiliation{Michigan Technological University, Houghton, MI, USA}

\author{J.M.~Figueira}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{P.~Filip}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Experimental Particle Physics, Karlsruhe, Germany}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{A.~Filip\v{c}i\v{c}}
\affiliation{Experimental Particle Physics Department, J.\ Stefan Institute, Ljubljana, Slovenia}
\affiliation{Center for Astrophysics and Cosmology (CAC), University of Nova Gorica, Nova Gorica, Slovenia}

\author{T.~Fitoussi}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{B.~Flaggs}
\affiliation{University of Delaware, Department of Physics and Astronomy, Bartol Research Institute, Newark, DE, USA}

\author{T.~Fodran}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}

\author{M.~Freitas}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{T.~Fujii}
\altaffiliation{now at Graduate School of Science, Osaka Metropolitan University, Osaka, Japan}
\affiliation{University of Chicago, Enrico Fermi Institute, Chicago, IL, USA}

\author{A.~Fuster}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\affiliation{Universidad Tecnol\'ogica Nacional -- Facultad Regional Buenos Aires, Buenos Aires, Argentina}

\author{C.~Galea}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}

\author{B.~Garc\'\i{}a}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), and Universidad Tecnol\'ogica Nacional -- Facultad Regional Mendoza (CONICET/CNEA), Mendoza, Argentina}

\author{C.~Gaudu}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{P.L.~Ghia}
\affiliation{CNRS/IN2P3, IJCLab, Universit\'e Paris-Saclay, Orsay, France}

\author{U.~Giaccari}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{F.~Gobbi}
\affiliation{Observatorio Pierre Auger, Malarg\"ue, Argentina}

\author{F.~Gollan}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{G.~Golup}
\affiliation{Centro At\'omico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), San Carlos de Bariloche, Argentina}

\author{M.~G\'omez Berisso}
\affiliation{Centro At\'omico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), San Carlos de Bariloche, Argentina}

\author{P.F.~G\'omez Vitale}
\affiliation{Observatorio Pierre Auger and Comisi\'on Nacional de Energ\'\i{}a At\'omica, Malarg\"ue, Argentina}

\author{J.P.~Gongora}
\affiliation{Observatorio Pierre Auger and Comisi\'on Nacional de Energ\'\i{}a At\'omica, Malarg\"ue, Argentina}

\author{J.M.~Gonz\'alez}
\affiliation{Centro At\'omico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), San Carlos de Bariloche, Argentina}

\author{N.~Gonz\'alez}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{D.~G\'ora}
\affiliation{Institute of Nuclear Physics PAN, Krakow, Poland}

\author{A.~Gorgi}
\affiliation{Osservatorio Astrofisico di Torino (INAF), Torino, Italy}
\affiliation{INFN, Sezione di Torino, Torino, Italy}

\author{M.~Gottowik}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{F.~Guarino}
\affiliation{Universit\`a di Napoli ``Federico II'', Dipartimento di Fisica ``Ettore Pancini'', Napoli, Italy}
\affiliation{INFN, Sezione di Napoli, Napoli, Italy}

\author{G.P.~Guedes}
\affiliation{Universidade Estadual de Feira de Santana, Feira de Santana, Brazil}

\author{E.~Guido}
\affiliation{Universit\"at Siegen, Department Physik -- Experimentelle Teilchenphysik, Siegen, Germany}

\author{L.~G\"ulzow}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{S.~Hahn}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Experimental Particle Physics, Karlsruhe, Germany}

\author{P.~Hamal}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{M.R.~Hampel}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{P.~Hansen}
\affiliation{IFLP, Universidad Nacional de La Plata and CONICET, La Plata, Argentina}

\author{V.M.~Harvey}
\affiliation{University of Adelaide, Adelaide, S.A., Australia}

\author{A.~Haungs}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{T.~Hebbeker}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{C.~Hojvat}
\altaffiliation{Fermi National Accelerator Laboratory, Fermilab, Batavia, IL, USA}

\author{J.R.~H\"orandel}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}
\affiliation{Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands}

\author{P.~Horvath}
\affiliation{Palacky University, Olomouc, Czech Republic}

\author{M.~Hrabovsk\'y}
\affiliation{Palacky University, Olomouc, Czech Republic}

\author{T.~Huege}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}
\affiliation{Vrije Universiteit Brussels, Brussels, Belgium}

\author{A.~Insolia}
\affiliation{Universit\`a di Catania, Dipartimento di Fisica e Astronomia ``Ettore Majorana``, Catania, Italy}
\affiliation{INFN, Sezione di Catania, Catania, Italy}

\author{P.G.~Isar}
\affiliation{Institute of Space Science, Bucharest-Magurele, Romania}

\author{P.~Janecek}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{V.~Jilek}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{J.~Jurysek}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{K.-H.~Kampert}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{B.~Keilhauer}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{A.~Khakurdikar}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}

\author{V.V.~Kizakke Covilakam}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{H.O.~Klages}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{M.~Kleifges}
\affiliation{Karlsruhe Institute of Technology (KIT), Institut f\"ur Prozessdatenverarbeitung und Elektronik, Karlsruhe, Germany}

\author{F.~Knapp}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Experimental Particle Physics, Karlsruhe, Germany}

\author{J.~K\"ohler}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{F.~Krieger}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{M.~Kubatova}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{N.~Kunka}
\affiliation{Karlsruhe Institute of Technology (KIT), Institut f\"ur Prozessdatenverarbeitung und Elektronik, Karlsruhe, Germany}

\author{B.L.~Lago}
\affiliation{Centro Federal de Educa\c{c}\~ao Tecnol\'ogica Celso Suckow da Fonseca, Petropolis, Brazil}

\author{N.~Langner}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{M.A.~Leigui de Oliveira}
\affiliation{Universidade Federal do ABC, Santo Andr\'e, SP, Brazil}

\author{Y.~Lema-Capeans}
\affiliation{Instituto Galego de F\'\i{}sica de Altas Enerx\'\i{}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain}

\author{A.~Letessier-Selvon}
\affiliation{Laboratoire de Physique Nucl\'eaire et de Hautes Energies (LPNHE), Sorbonne Universit\'e, Universit\'e de Paris, CNRS-IN2P3, Paris, France}

\author{I.~Lhenry-Yvon}
\affiliation{CNRS/IN2P3, IJCLab, Universit\'e Paris-Saclay, Orsay, France}

\author{L.~Lopes}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{J.P.~Lundquist}
\affiliation{Center for Astrophysics and Cosmology (CAC), University of Nova Gorica, Nova Gorica, Slovenia}

\author{A.~Machado Payeras}
\affiliation{Universidade Estadual de Campinas (UNICAMP), IFGW, Campinas, SP, Brazil}

\author{D.~Mandat}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{B.C.~Manning}
\affiliation{University of Adelaide, Adelaide, S.A., Australia}

\author{P.~Mantsch}
\altaffiliation{Fermi National Accelerator Laboratory, Fermilab, Batavia, IL, USA}

\author{F.M.~Mariani}
\affiliation{Universit\`a di Milano, Dipartimento di Fisica, Milano, Italy}
\affiliation{INFN, Sezione di Milano, Milano, Italy}

\author{A.G.~Mariazzi}
\affiliation{IFLP, Universidad Nacional de La Plata and CONICET, La Plata, Argentina}

\author{I.C.~Mari\c{s}}
\affiliation{Universit\'e Libre de Bruxelles (ULB), Brussels, Belgium}

\author{G.~Marsella}
\affiliation{Universit\`a di Palermo, Dipartimento di Fisica e Chimica ''E.\ Segr\`e'', Palermo, Italy}
\affiliation{INFN, Sezione di Catania, Catania, Italy}

\author{D.~Martello}
\affiliation{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{S.~Martinelli}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{O.~Mart\'\i{}nez Bravo}
\affiliation{Benem\'erita Universidad Aut\'onoma de Puebla, Puebla, M\'exico}

\author{M.A.~Martins}
\affiliation{Instituto Galego de F\'\i{}sica de Altas Enerx\'\i{}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain}

\author{H.-J.~Mathes}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{J.~Matthews}
\altaffiliation{Louisiana State University, Baton Rouge, LA, USA}

\author{G.~Matthiae}
\affiliation{Universit\`a di Roma ``Tor Vergata'', Dipartimento di Fisica, Roma, Italy}
\affiliation{INFN, Sezione di Roma ``Tor Vergata'', Roma, Italy}

\author{E.~Mayotte}
\affiliation{Colorado School of Mines, Golden, CO, USA}

\author{S.~Mayotte}
\affiliation{Colorado School of Mines, Golden, CO, USA}

\author{P.O.~Mazur}
\altaffiliation{Fermi National Accelerator Laboratory, Fermilab, Batavia, IL, USA}

\author{G.~Medina-Tanco}
\affiliation{Universidad Nacional Aut\'onoma de M\'exico, M\'exico, D.F., M\'exico}

\author{J.~Meinert}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{D.~Melo}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{A.~Menshikov}
\affiliation{Karlsruhe Institute of Technology (KIT), Institut f\"ur Prozessdatenverarbeitung und Elektronik, Karlsruhe, Germany}

\author{C.~Merx}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{S.~Michal}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{M.I.~Micheletti}
\affiliation{Instituto de F\'\i{}sica de Rosario (IFIR) -- CONICET/U.N.R.\ and Facultad de Ciencias Bioqu\'\i{}micas y Farmac\'euticas U.N.R., Rosario, Argentina}

\author{L.~Miramonti}
\affiliation{Universit\`a di Milano, Dipartimento di Fisica, Milano, Italy}
\affiliation{INFN, Sezione di Milano, Milano, Italy}

\author{S.~Mollerach}
\affiliation{Centro At\'omico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), San Carlos de Bariloche, Argentina}

\author{F.~Montanet}
\affiliation{Univ.\ Grenoble Alpes, CNRS, Grenoble Institute of Engineering Univ.\ Grenoble Alpes, LPSC-IN2P3, 38000 Grenoble, France}

\author{L.~Morejon}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{K.~Mulrey}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}
\affiliation{Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands}

\author{R.~Mussa}
\affiliation{INFN, Sezione di Torino, Torino, Italy}

\author{W.M.~Namasaka}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{S.~Negi}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{L.~Nellen}
\affiliation{Universidad Nacional Aut\'onoma de M\'exico, M\'exico, D.F., M\'exico}

\author{K.~Nguyen}
\affiliation{Michigan Technological University, Houghton, MI, USA}

\author{G.~Nicora}
\affiliation{Laboratorio Atm\'osfera -- Departamento de Investigaciones en L\'aseres y sus Aplicaciones -- UNIDEF (CITEDEF-CONICET), Argentina}

\author{M.~Niechciol}
\affiliation{Universit\"at Siegen, Department Physik -- Experimentelle Teilchenphysik, Siegen, Germany}

\author{D.~Nitz}
\affiliation{Michigan Technological University, Houghton, MI, USA}

\author{D.~Nosek}
\affiliation{Charles University, Faculty of Mathematics and Physics, Institute of Particle and Nuclear Physics, Prague, Czech Republic}

\author{V.~Novotny}
\affiliation{Charles University, Faculty of Mathematics and Physics, Institute of Particle and Nuclear Physics, Prague, Czech Republic}

\author{L.~No\v{z}ka}
\affiliation{Palacky University, Olomouc, Czech Republic}

\author{A.~Nucita}
\affiliation{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{L.A.~N\'u\~nez}
\affiliation{Universidad Industrial de Santander, Bucaramanga, Colombia}

\author{C.~Oliveira}
\affiliation{Universidade de S\~ao Paulo, Instituto de F\'\i{}sica de S\~ao Carlos, S\~ao Carlos, SP, Brazil}

\author{M.~Palatka}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{J.~Pallotta}
\affiliation{Laboratorio Atm\'osfera -- Departamento de Investigaciones en L\'aseres y sus Aplicaciones -- UNIDEF (CITEDEF-CONICET), Argentina}

\author{S.~Panja}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{G.~Parente}
\affiliation{Instituto Galego de F\'\i{}sica de Altas Enerx\'\i{}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain}

\author{T.~Paulsen}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{J.~Pawlowsky}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{M.~Pech}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{J.~P\c{e}kala}
\affiliation{Institute of Nuclear Physics PAN, Krakow, Poland}

\author{R.~Pelayo}
\affiliation{Unidad Profesional Interdisciplinaria en Ingenier\'\i{}a y Tecnolog\'\i{}as Avanzadas del Instituto Polit\'ecnico Nacional (UPIITA-IPN), M\'exico, D.F., M\'exico}

\author{V.~Pelgrims}
\affiliation{Universit\'e Libre de Bruxelles (ULB), Brussels, Belgium}

\author{L.A.S.~Pereira}
\affiliation{Universidade Federal de Campina Grande, Centro de Ciencias e Tecnologia, Campina Grande, Brazil}

\author{E.E.~Pereira Martins}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Experimental Particle Physics, Karlsruhe, Germany}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{C.~P\'erez Bertolli}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{L.~Perrone}
\affiliation{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{S.~Petrera}
\affiliation{Gran Sasso Science Institute, L'Aquila, Italy}
\affiliation{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}

\author{C.~Petrucci}
\affiliation{Universit\`a dell'Aquila, Dipartimento di Scienze Fisiche e Chimiche, L'Aquila, Italy}

\author{T.~Pierog}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{M.~Pimenta}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{M.~Platino}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{B.~Pont}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}

\author{M.~Pothast}
\affiliation{Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}

\author{M.~Pourmohammad Shahvar}
\affiliation{Universit\`a di Palermo, Dipartimento di Fisica e Chimica ''E.\ Segr\`e'', Palermo, Italy}
\affiliation{INFN, Sezione di Catania, Catania, Italy}

\author{P.~Privitera}
\affiliation{University of Chicago, Enrico Fermi Institute, Chicago, IL, USA}

\author{M.~Prouza}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{S.~Querchfeld}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{J.~Rautenberg}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{D.~Ravignani}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{J.V.~Reginatto Akim}
\affiliation{Universidade Estadual de Campinas (UNICAMP), IFGW, Campinas, SP, Brazil}

\author{A.~Reuzki}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{J.~Ridky}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{F.~Riehn}
\affiliation{Instituto Galego de F\'\i{}sica de Altas Enerx\'\i{}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain}

\author{M.~Risse}
\affiliation{Universit\"at Siegen, Department Physik -- Experimentelle Teilchenphysik, Siegen, Germany}

\author{V.~Rizi}
\affiliation{Universit\`a dell'Aquila, Dipartimento di Scienze Fisiche e Chimiche, L'Aquila, Italy}
\affiliation{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}

\author{E.~Rodriguez}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{J.~Rodriguez Rojo}
\affiliation{Observatorio Pierre Auger and Comisi\'on Nacional de Energ\'\i{}a At\'omica, Malarg\"ue, Argentina}

\author{M.J.~Roncoroni}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{S.~Rossoni}
\affiliation{Universit\"at Hamburg, II.\ Institut f\"ur Theoretische Physik, Hamburg, Germany}

\author{M.~Roth}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{E.~Roulet}
\affiliation{Centro At\'omico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), San Carlos de Bariloche, Argentina}

\author{A.C.~Rovero}
\affiliation{Instituto de Astronom\'\i{}a y F\'\i{}sica del Espacio (IAFE, CONICET-UBA), Buenos Aires, Argentina}

\author{A.~Saftoiu}
\affiliation{``Horia Hulubei'' National Institute for Physics and Nuclear Engineering, Bucharest-Magurele, Romania}

\author{M.~Saharan}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}

\author{F.~Salamida}
\affiliation{Universit\`a dell'Aquila, Dipartimento di Scienze Fisiche e Chimiche, L'Aquila, Italy}
\affiliation{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}

\author{H.~Salazar}
\affiliation{Benem\'erita Universidad Aut\'onoma de Puebla, Puebla, M\'exico}

\author{G.~Salina}
\affiliation{INFN, Sezione di Roma ``Tor Vergata'', Roma, Italy}

\author{P.~Sampathkumar}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{J.D.~Sanabria Gomez}
\affiliation{Universidad Industrial de Santander, Bucaramanga, Colombia}

\author{F.~S\'anchez}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{E.M.~Santos}
\affiliation{Universidade de S\~ao Paulo, Instituto de F\'\i{}sica, S\~ao Paulo, SP, Brazil}

\author{E.~Santos}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{F.~Sarazin}
\affiliation{Colorado School of Mines, Golden, CO, USA}

\author{R.~Sarmento}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{R.~Sato}
\affiliation{Observatorio Pierre Auger and Comisi\'on Nacional de Energ\'\i{}a At\'omica, Malarg\"ue, Argentina}

\author{C.M.~Sch\"afer}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Experimental Particle Physics, Karlsruhe, Germany}

\author{V.~Scherini}
\affiliation{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{H.~Schieler}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{M.~Schimassek}
\affiliation{CNRS/IN2P3, IJCLab, Universit\'e Paris-Saclay, Orsay, France}

\author{M.~Schimp}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{D.~Schmidt}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{O.~Scholten}
\altaffiliation{also at Kapteyn Institute, University of Groningen, Groningen, The Netherlands}
\affiliation{Vrije Universiteit Brussels, Brussels, Belgium}

\author{H.~Schoorlemmer}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}
\affiliation{Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands}

\author{P.~Schov\'anek}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{F.G.~Schr\"oder}
\affiliation{University of Delaware, Department of Physics and Astronomy, Bartol Research Institute, Newark, DE, USA}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{J.~Schulte}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{T.~Schulz}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{S.J.~Sciutto}
\affiliation{IFLP, Universidad Nacional de La Plata and CONICET, La Plata, Argentina}

\author{M.~Scornavacche}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{A.~Sedoski}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{A.~Segreto}
\affiliation{Istituto di Astrofisica Spaziale e Fisica Cosmica di Palermo (INAF), Palermo, Italy}
\affiliation{INFN, Sezione di Catania, Catania, Italy}

\author{S.~Sehgal}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{S.U.~Shivashankara}
\affiliation{Center for Astrophysics and Cosmology (CAC), University of Nova Gorica, Nova Gorica, Slovenia}

\author{G.~Sigl}
\affiliation{Universit\"at Hamburg, II.\ Institut f\"ur Theoretische Physik, Hamburg, Germany}

\author{K.~Simkova}
\affiliation{Vrije Universiteit Brussels, Brussels, Belgium}
\affiliation{Universit\'e Libre de Bruxelles (ULB), Brussels, Belgium}

\author{F.~Simon}
\affiliation{Karlsruhe Institute of Technology (KIT), Institut f\"ur Prozessdatenverarbeitung und Elektronik, Karlsruhe, Germany}

\author{R.~\v{S}m\'\i{}da}
\affiliation{University of Chicago, Enrico Fermi Institute, Chicago, IL, USA}

\author{P.~Sommers}
\altaffiliation{Pennsylvania State University, University Park, PA, USA}

\author{R.~Squartini}
\affiliation{Observatorio Pierre Auger, Malarg\"ue, Argentina}

\author{M.~Stadelmaier}
\affiliation{INFN, Sezione di Milano, Milano, Italy}
\affiliation{Universit\`a di Milano, Dipartimento di Fisica, Milano, Italy}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{S.~Stani\v{c}}
\affiliation{Center for Astrophysics and Cosmology (CAC), University of Nova Gorica, Nova Gorica, Slovenia}

\author{J.~Stasielak}
\affiliation{Institute of Nuclear Physics PAN, Krakow, Poland}

\author{P.~Stassi}
\affiliation{Univ.\ Grenoble Alpes, CNRS, Grenoble Institute of Engineering Univ.\ Grenoble Alpes, LPSC-IN2P3, 38000 Grenoble, France}

\author{S.~Str\"ahnz}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Experimental Particle Physics, Karlsruhe, Germany}

\author{M.~Straub}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{T.~Suomij\"arvi}
\affiliation{Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, Orsay, France}

\author{A.D.~Supanitsky}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{Z.~Svozilikova}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{Z.~Szadkowski}
\affiliation{University of \L{}\'od\'z, Faculty of High-Energy Astrophysics,\L{}\'od\'z, Poland}

\author{F.~Tairli}
\affiliation{University of Adelaide, Adelaide, S.A., Australia}

\author{A.~Tapia}
\affiliation{Universidad de Medell\'\i{}n, Medell\'\i{}n, Colombia}

\author{C.~Taricco}
\affiliation{Universit\`a Torino, Dipartimento di Fisica, Torino, Italy}
\affiliation{INFN, Sezione di Torino, Torino, Italy}

\author{C.~Timmermans}
\affiliation{Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}

\author{O.~Tkachenko}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{P.~Tobiska}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{C.J.~Todero Peixoto}
\affiliation{Universidade de S\~ao Paulo, Escola de Engenharia de Lorena, Lorena, SP, Brazil}

\author{B.~Tom\'e}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{Z.~Torr\`es}
\affiliation{Univ.\ Grenoble Alpes, CNRS, Grenoble Institute of Engineering Univ.\ Grenoble Alpes, LPSC-IN2P3, 38000 Grenoble, France}

\author{A.~Travaini}
\affiliation{Observatorio Pierre Auger, Malarg\"ue, Argentina}

\author{P.~Travnicek}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{M.~Tueros}
\affiliation{IFLP, Universidad Nacional de La Plata and CONICET, La Plata, Argentina}

\author{M.~Unger}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{R.~Uzeiroska}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{L.~Vaclavek}
\affiliation{Palacky University, Olomouc, Czech Republic}

\author{M.~Vacula}
\affiliation{Palacky University, Olomouc, Czech Republic}

\author{J.F.~Vald\'es Galicia}
\affiliation{Universidad Nacional Aut\'onoma de M\'exico, M\'exico, D.F., M\'exico}

\author{L.~Valore}
\affiliation{Universit\`a di Napoli ``Federico II'', Dipartimento di Fisica ``Ettore Pancini'', Napoli, Italy}
\affiliation{INFN, Sezione di Napoli, Napoli, Italy}

\author{E.~Varela}
\affiliation{Benem\'erita Universidad Aut\'onoma de Puebla, Puebla, M\'exico}

\author{V.~Va\v{s}\'\i{}\v{c}kov\'a}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{A.~V\'asquez-Ram\'\i{}rez}
\affiliation{Universidad Industrial de Santander, Bucaramanga, Colombia}

\author{D.~Veberi\v{c}}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{I.D.~Vergara Quispe}
\affiliation{IFLP, Universidad Nacional de La Plata and CONICET, La Plata, Argentina}

\author{V.~Verzi}
\affiliation{INFN, Sezione di Roma ``Tor Vergata'', Roma, Italy}

\author{J.~Vicha}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{J.~Vink}
\affiliation{Universiteit van Amsterdam, Faculty of Science, Amsterdam, The Netherlands}

\author{S.~Vorobiov}
\affiliation{Center for Astrophysics and Cosmology (CAC), University of Nova Gorica, Nova Gorica, Slovenia}

\author{C.~Watanabe}
\affiliation{Universidade Federal do Rio de Janeiro, Instituto de F\'\i{}sica, Rio de Janeiro, RJ, Brazil}

\author{A.A.~Watson}
\altaffiliation{School of Physics and Astronomy, University of Leeds, Leeds, United Kingdom}

\author{A.~Weindl}
\affiliation{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}

\author{M.~Weitz}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{L.~Wiencke}
\affiliation{Colorado School of Mines, Golden, CO, USA}

\author{H.~Wilczy\'nski}
\affiliation{Institute of Nuclear Physics PAN, Krakow, Poland}

\author{D.~Wittkowski}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{B.~Wundheiler}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{B.~Yue}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{A.~Yushkov}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{O.~Zapparrata}
\affiliation{Universit\'e Libre de Bruxelles (ULB), Brussels, Belgium}

\author{E.~Zas}
\affiliation{Instituto Galego de F\'\i{}sica de Altas Enerx\'\i{}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain}

\author{D.~Zavrtanik}
\affiliation{Center for Astrophysics and Cosmology (CAC), University of Nova Gorica, Nova Gorica, Slovenia}
\affiliation{Experimental Particle Physics Department, J.\ Stefan Institute, Ljubljana, Slovenia}

\author{M.~Zavrtanik}
\affiliation{Experimental Particle Physics Department, J.\ Stefan Institute, Ljubljana, Slovenia}
\affiliation{Center for Astrophysics and Cosmology (CAC), University of Nova Gorica, Nova Gorica, Slovenia}

\collaboration{0}{The Pierre Auger Collaboration}
\email{spokespersons@auger.org}

